On the Utility of Buffers in Pick-n-Swap Based Lattice Rearrangement

We investigate the utility of employing multiple buffers in solving a class of rearrangement problems with pick-n-swap manipulation primitives. In this problem, objects stored randomly in a lattice are to be sorted using a robot arm with k>=1 swap spaces or buffers, capable of holding up to k objects on its end-effector simultaneously. On the structural side, we show that the addition of each new buffer brings diminishing returns in saving the end-effector travel distance while holding the total number of pick-n-swap operations at the minimum. This is due to an interesting recursive cycle structure in random m-permutation, where the largest cycle covers over 60% of objects. On the algorithmic side, we propose fast algorithms for 1D and 2D lattice rearrangement problems that can effectively use multiple buffers to boost solution optimality. Numerical experiments demonstrate the efficiency and scalability of our methods, as well as confirm the diminishing return structure as more buffers are employed.

==> 00-contents.tex <==
\begin{enumerate}
    \item Properties
        \begin{enumerate}
            \item Observation of multi-buffer pick-and-swaps (in/inter-cycle, in/inter-cycle group).
            \begin{enumerate}
                \item Paralleling pick-and-swaps in the same cycle will increase $\#$ swaps.
                \item Inter-group tasks can be considered individually.
            \end{enumerate}
            \item Solution pattern when $\#$ swaps is minimized: cycle-buffer assignment and cycle ordering.
            \begin{enumerate}
                \item Each cycle is dealt with by only one buffer.
                \item A stack-like structure of cycles for each buffer.
            \end{enumerate}
            \item The expectation of the largest cycle is lower bounded by 0.547 m.
            \item According to the 100-prisoners problem, there is a around 69$\%$ possibility to have a dominating cycle that has more objects than the total number of objects in the other cycles.
            \item Around $20\%$ reduction of distance cost when the second buffer is available. Much less improvement when the third buffer is available.
        \end{enumerate}
    \item Computing optimal distance cost with min($\#$ swaps)
    \begin{enumerate}
        \item When $\#$ cycle in a cycle group $\leq$ $\#$ buffers, $O(kn^{2k-1})$ with DP.
        \begin{enumerate}
            \item In the 1D case, we can start from the min(cycle group) without loss of optimality. 
        \end{enumerate}
        \item When $\#$ cycle in a cycle group $>$ $\#$ buffers, current exact algorithm:
        \begin{enumerate}
            \item A recursive generator for cycle-buffer assignment and cycle ordering
            \item enumerate breaking points for cycle switching
            \item $O(kn^k)$ for $k$-buffer task sequence merging with DP
        \end{enumerate}
    \end{enumerate}
    \item Algorithms for general optimal objective functions
    \begin{enumerate}
        \item MCTS
        \begin{enumerate}
            \item MCTS with reweighting UCB
        \end{enumerate}
    \end{enumerate}
    \item Potential directions to work on
    \begin{enumerate}
        \item Applying the idea of ``finite horizon'' to algorithms?
        \item Expected distance saving with $k$-buffers?
        \item Additional Observations to improve the exact algorithm
    \end{enumerate}
\end{enumerate}

